Tails Tell Tales: Chapter-Wide Manga Transcriptions with Character Names

Enabling engagement of manga by visually impaired individuals presents a significant challenge due to its inherently visual nature. With the goal of fostering accessibility, this paper aims to generate a dialogue transcript of a complete manga chapter, entirely automatically, with a particular emphasis on ensuring narrative consistency. This entails identifying (i) what is being said, i.e., detecting the texts on each page and classifying them into essential vs non-essential, and (ii) who is saying it, i.e., attributing each dialogue to its speaker, while ensuring the same characters are named consistently throughout the chapter. To this end, we introduce: (i) Magiv2, a model that is capable of generating high-quality chapter-wide manga transcripts with named characters and significantly higher precision in speaker diarisation over prior works; (ii) an extension of the PopManga evaluation dataset, which now includes annotations for speech-bubble tail boxes, associations of text to corresponding tails, classifications of text as essential or non-essential, and the identity for each character box; and (iii) a new character bank dataset, which comprises over 11K characters from 76 manga series, featuring 11.5K exemplar character images in total, as well as a list of chapters in which they appear. The code, trained model, and both datasets can be found at: https://github.com/ragavsachdeva/magi

==> tables/popmanga-test-x.tex <==
{
\setlength{\tabcolsep}{3pt}
\begin{table}[!t]
\fontsize{7.5pt}{10pt}\selectfont
\centering
\caption{\textbf{Difference in annotations between PopManga and \pmx.} Note that \pmx is an extension of PopManga, thus containing all annotations of PopManga.}
% Default setting is marked in \colorbox{grey_cell}{gray}.
\vspace{-3mm}
\begin{tabular}{l|c}
& annotation type\\ \shline
\rowcolor{grey_cell}
PopManga & character box, text box, per-page character cluster, speaker association\\
\pmx (Ours) & tail box, text-tail association, text categories
\end{tabular}
\label{tab:popmanga-test-x}
\end{table}
}

